What is a Labor Market? Classifying Workers and Jobs Using Network Theory

This paper develops a new data-driven approach to characterizing latent worker skill and job task heterogeneity by applying an empirical tool from network theory to large-scale Brazilian administrative data on worker--job matching. We microfound this tool using a standard equilibrium model of workers matching with jobs according to comparative advantage. Our classifications identify important dimensions of worker and job heterogeneity that standard classifications based on occupations and sectors miss. The equilibrium model based on our classifications more accurately predicts wage changes in response to the 2016 Olympics than a model based on occupations and sectors. Additionally, for a large simulated shock to demand for workers, we show that reduced form estimates of the effects of labor market shock exposure on workers' earnings are nearly 4 times larger when workers and jobs are classified using our classifications as opposed to occupations and sectors.

==> ImportedResults/occ_counts_iota360_presentation.tex <==
\begin{tabularx}{\textwidth}{llr}
\toprule
{Occ-6}&{Occupation Name}&{Share} \tabularnewline
\midrule\addlinespace[1.5ex]
333110&Course Instructor&0.15 \tabularnewline
224120&Personal trainer&0.11 \tabularnewline
231315&Physical Education Teacher in Primary School&0.08 \tabularnewline
224125&Coach (except for soccer)&0.06 \tabularnewline
234410&Physical Education Teacher in Higher Education \hspace{2.12cm} &0.05 \tabularnewline
224105&Fitness monitor&0.05 \tabularnewline
333115&Teacher (with High School degree)&0.05 \tabularnewline
234520&Education Teacher (with College degree) & 0.03 \tabularnewline
371410&Recreational Activities Coordinator&0.03 \tabularnewline
377105&Professional Athlete (various modalities)&0.02 \tabularnewline
\bottomrule \addlinespace[1.5ex]
\end{tabularx}



==> ImportedResults/occ_counts_iota557_presentation.tex <==
\begin{tabularx}{\textwidth}{llr}
\toprule
{Occ-6}&{Occupation Name}&{Share} \tabularnewline
\midrule\addlinespace[1.5ex]
331205&Elementary School Teacher &0.07 \tabularnewline
333110&Course Instructor&0.07 \tabularnewline
231210&Elementary School Teacher (1st to 4th grade)&0.06 \tabularnewline
231205&Young and Adult Teacher teaching elementary school content \hspace{.3cm} &0.06 \tabularnewline
232115&High School Teacher&0.05 \tabularnewline
234616&English Teacher&0.04 \tabularnewline
333115&Teacher of Free Courses&0.03 \tabularnewline
231305&Elementary School Science and Math Teacher&0.03 \tabularnewline
331105&Kindergarten Teacher &0.02 \tabularnewline
231310&Art Teacher in Elementary School&0.02 \tabularnewline
\bottomrule \addlinespace[1.5ex]
\end{tabularx}



==> Results/nmi.tex <==
iota & gamma & 0.466
iota & cbo2002\_first & 0.21
iota & clas\_cnae20\_first & 0.193
gamma & cbo2002\_first & 0.198
gamma & clas\_cnae20\_first & 0.197
cbo2002\_first & clas\_cnae20\_first & 0.412


==> tex/tikz_ADH_adapted.tex <==

\definecolor{myblue}{RGB}{80,80,160}
\definecolor{mygreen}{RGB}{80,160,80}

\begin{tikzpicture}[thick,
every node/.style={draw,circle},
isnode/.style={fill=orange},
gsnode/.style={fill=mygreen},
ssnode/.style={fill=myblue},
every fit/.style={rectangle,draw,inner sep=1pt, text height=2cm},
->,shorten >= 3pt,shorten <= 3pt
]

% the vertices of S
\begin{scope}[xshift=1cm, start chain=going right,node distance=7mm]
\foreach \i in {1,2,3}
\node[ssnode,on chain] (s\i)  {};
\end{scope}

% the vertices of G
\begin{scope}[xshift=1cm,yshift=-2cm,start chain=going right,node distance=7mm]
\foreach \i in {4,5,...,6}
\node[gsnode,on chain] (g\i)  {};
\end{scope}

% the vertices of I
\begin{scope}[xshift=0.5cm,yshift=-4cm,start chain=going right,node distance=7mm]
\foreach \i in {9,10,...,12}
\node[isnode,on chain] (i\i)  {};
\end{scope}

% the set S
\node [myblue, fit=(s1) (s3), label={[text=myblue]right:$S$}] {};
% the set G
\node [mygreen,fit=(g4) (g6),label={[text=mygreen]right:$\g$}] {};
% the set I
\node [orange,fit=(i9) (i12),label={[text=orange]right:$\i$}] {};

%{node[label={[font=\small,text=blue]30:$-1$}] {10}}

% the edges
\draw (g4) -- (s1);
\draw (g5) -- (s2);
\draw (g6) -- (s3);
\draw (i9)  -- (g4);
\draw (i10) -- (g4);
\draw (i11) -- (g4);
\draw (i12) -- (g4);
\draw (i9)  -- (g5);
\draw (i10) -- (g5);
\draw (i11) -- (g5);
\draw (i12) -- (g5);
\draw (i9)  -- (g6);
\draw (i10) -- (g6);
\draw (i11) -- (g6);
\draw (i12) -- (g6);
\end{tikzpicture}


==> tex/tikz_ADH_adapted_occ2.tex <==

\definecolor{myblue}{RGB}{80,80,160}
\definecolor{mygreen}{RGB}{80,160,80}

\begin{tikzpicture}[thick,
every node/.style={draw,circle},
isnode/.style={fill=orange},
gsnode/.style={fill=mygreen},
ssnode/.style={fill=myblue},
every fit/.style={rectangle,draw,inner sep=1pt, text height=2cm},
->,shorten >= 3pt,shorten <= 3pt
]

% the vertices of S
\begin{scope}[xshift=1cm, start chain=going right,node distance=7mm]
\foreach \i in {1,2,3}
\node[ssnode,on chain] (s\i)  {};
\end{scope}

% the vertices of G
\begin{scope}[xshift=1cm,yshift=-2cm,start chain=going right,node distance=7mm]
\foreach \i in {4,5,...,6}
\node[gsnode,on chain] (g\i)  {};
\end{scope}

% the vertices of I
\begin{scope}[xshift=0.5cm,yshift=-4cm,start chain=going right,node distance=7mm]
\foreach \i in {9,10,...,12}
\node[isnode,on chain] (i\i)  {};
\end{scope}

% the set S
\node [myblue, fit=(s1) (s3), label={[text=myblue]right:$S$}] {};
% the set G
\node [mygreen,fit=(g4) (g6),label={[text=mygreen]right:$\g$}] {};
% the set I
\node [orange,fit=(i9) (i12),label={[text=orange]right:Occ2}] {};

%{node[label={[font=\small,text=blue]30:$-1$}] {10}}

% the edges
\draw (g4) -- (s1);
\draw (g5) -- (s2);
\draw (g6) -- (s3);
\draw (i9)  -- (g4);
\draw (i10) -- (g4);
\draw (i11) -- (g4);
\draw (i12) -- (g4);
\draw (i9)  -- (g5);
\draw (i10) -- (g5);
\draw (i11) -- (g5);
\draw (i12) -- (g5);
\draw (i9)  -- (g6);
\draw (i10) -- (g6);
\draw (i11) -- (g6);
\draw (i12) -- (g6);
\end{tikzpicture}

